Computing Join Queries with Functional Dependencies

Recently, Gottlob, Lee, Valiant, and Valiant (GLVV) presented an output size bound for join queries with functional dependencies (FD), based on a linear program on polymatroids. GLVV bound strictly generalizes the bound of Atserias, Grohe and Marx (AGM) for queries with no FD, in which case there are known algorithms running within AGM bound and thus are worst-case optimal. A main result of this paper is an algorithm for computing join queries with FDs, running within GLVV bound up to a poly-log factor. In particular, our algorithm is worst-case optimal for any query where the GLVV bound is tight. As an unexpected by-product, our algorithm manages to solve a harder problem, where (some) input relations may have prescribed maximum degree bounds, of which both functional dependencies and cardinality bounds are special cases. We extend Gottlob et al. framework by replacing all variable subsets with the lattice of closed sets (under the given FDs). This gives us new insights into the structure of the worst-case bound and worst-case instances. While it is still open whether GLVV bound is tight in general, we show that it is tight on distributive lattices and some other simple lattices. Distributive lattices capture a strict superset of queries with no FD and with simple FDs. We also present two simpler algorithms which are also worst-case optimal on distributive lattices within a single-$\log$ factor, but they do not match GLVV bound on a general lattice. Our algorithms are designed based on a novel principle: we turn a proof of a polymatroid-based output size bound into an algorithm.

==> proof-systems.tex <==
 This follows from a simple and elegant result from the theory
of generalized inequalities~\cite[Ch.2]{boyd:vandenberghe:2004},
briefly reviewed here.  Denoting $K
\defeq \setof{h}{Mh \geq 0}$, and it's dual $K^* \defeq \setof{d}{d^T
  h \leq 0, \forall h \in K}$, \footnote{These definitions are similar
  to those of a {\em cone} and a {\em dual cone}
  in~\cite[Ch.2]{boyd:vandenberghe:2004}, except that we used $\leq 0$
  instead of the standard $\geq 0$.} we have:

\begin{prop} \label{prop:ineq} \cite{boyd:vandenberghe:2004} Let
  $d\geq 0$.  Then $\forall h\geq 0, Mh \leq 0$ implies $d^T h \leq 0$
  iff there exists $s \geq 0$ such that $d^T \leq s^T M$.
\end{prop}

\begin{proof} We briefly sketch the proof, for completeness. For the
  ``if'' direction, assume $d^T \leq s^T M$: if $Mh \leq 0$ then $0
  \geq s^T M h \geq d^T h$ proving the claim.  For ``only if'',
  consider the linear program $\max(d^T h), Mh \leq 0$; its optimal
  value is $\leq 0$, because $Mh \leq 0$ implies $d^T h \leq 0$.  Then
  the dual, $\min 0, s^T M \geq d$, must have a feasible solution $s$,
  otherwise its optimal is $+\infty$, proving the claim.
\end{proof}





For a simple illustration, consider the triangle query
$Q=R(x,y),S(y,z),T(z,x)$, without any functional dependencies.  Its
lattice is the Boolean algebra $2^{\set{x,y,z}}$.  The following are
examples of output inequalities:
\begin{eqnarray*}
   h(xy)+h(yz)+h(zx) &\geq & 2h(\hat 1) \\
   h(xy)+h(yz) &\geq & h(\hat 1)
\end{eqnarray*}
The first is proven using two sub-modularity steps: $h(xy)+h(yz) \geq
h(xyz)+h(y)=h(\hat 1) + h(y)$, and $h(y)+h(zx)\geq h(\hat 1) + h(\hat
0)$.  The corresponding vector $s$ in Prop.~\ref{prop:ineq} is
$s_{xy,yz}=s_{y,zx}=1$ with the rest 0.  To see the connection to the
optimal LLP, assume $n_R=n_S=n_T=6$; then $h^*(\hat 1) = 9$, which can
be derived from the first inequality, $2h(\hat 1) \leq n_R+n_S+n_T$.
On the other hand, if $n_R=2$, $n_S=n_T=5$, then $h^*(\hat 1) = 7$
which can be derived from the second inequality $h(\hat 1) \leq
n_R+n_S$.

